Learning with Unlearning: Synaptic Role Partitioning for Simultaneous Continual Learning and Machine Unlearning

Continual Learning (CL) asks a model to acquire new knowledge without forgetting what it already knows. Machine Unlearning (MU) asks it to destroy specific knowledge without damaging the rest. The challenge is integrating them in the same system; the two objectives pull on the same weights, and an edit made for one harms the other. To address this, we propose Learning with Unlearning (LwU), a unified framework that resolves the conflict where it occurs: at the individual synapse. LwU scores every weight twice, once against the data to keep and once against the data to delete, and partitions the network into four zones with separate update rules. Weights that only require retention are frozen. Weights that only require deletion are cleared and returned to the network as free capacity. Contested weights take a gradient-ascent step projected orthogonally to the retention gradient. The remaining capacity learns the incoming task by a privileged teacher via self-distillation. Deletion is served post hoc, and no retraining is required. Across both CL and MU jobs, LwU outperforms or matches the strongest baseline. Its real-world practicality has been demonstrated on the Physical Artificial Intelligence (PAI) dataset we conducted. Additionally, in the image generation task and in removing dangerous content, it outperformed the closest baseline, as shown in Fig.1.

==> new_results_only.tex <==
\subsection{New Interleaved Continual Learning and Machine Unlearning Results}\label{sec:new_joint_clmu}
All new interleaved evaluations in this subsection use Split CIFAR-100 and ResNet-18 in Task-IL. The five-task setting comprises five tasks of 20 classes, three seeds, and deletion of the first class of task 1 after task 3, followed by learning tasks 4--5. $F_{\mathrm{del}}$ and $F_{\mathrm{end}}$ measure accuracy on the deleted class immediately after deletion and after the final task; for class deletion, the Retrain reference is zero. These experiments examine an interleaved lifecycle rather than inferring joint behavior from standalone CL and MU metrics.

In composed baselines the continual learner completes tasks 1--3, an MU method edits the model, and continual learning resumes; when relevant, the LwF teacher and EWC anchor are reset to the edited model. CLPU-DER++ requires advance knowledge of the future forget class to isolate its model copy. Storage is measured at the deletion request. Default $\mathcal{D}'_r$ is a sampled 10\% of retained training images from tasks 1--3 (2,480 images); LwU maintains no replay buffer during sequential learning but has access to these images at deletion. An additional experiment removes this older-task access.

\begin{table*}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\caption{Five-task joint CL--MU comparison. Means $\pm$ standard deviations over three seeds. The request-time variant uses no images from tasks 1--2; CLPU-DER++ requires advance knowledge of the deleted class.}
\label{tab:new_joint_baselines}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{lccccc}
\toprule
Method & Stored images at the request & ACC $\uparrow$ & BWT $\uparrow$ & $F_{\mathrm{del}}$ $\downarrow$ & $F_{\mathrm{end}}$ $\downarrow$ \\
\midrule
Retrain (never sees $c_f$) & -- & $71.75\pm0.73$ & $-2.95\pm0.11$ & -- & $0.00\pm0.00$ \\
LwF + SSD$^\dagger$ & $\mathcal{D}'_r$ (2,480) & $64.53\pm9.76$ & $-13.68\pm13.82$ & $30.89\pm36.59$ & $32.82\pm38.22$ \\
LwF + SalUn & $\mathcal{D}'_r$ (2,480) & $69.94\pm2.45$ & $-7.24\pm0.83$ & $4.42\pm3.84$ & $2.26\pm2.68$ \\
EWC + SCRUB & $\mathcal{D}'_r$ (2,480) & $66.90\pm0.89$ & $0.10\pm0.92$ & $68.87\pm25.75$ & $65.54\pm29.65$ \\
UniCLUN & buffer (1,000) + $\mathcal{D}'_r$ & $49.62\pm10.16$ & $-26.19\pm6.25$ & $28.12\pm23.45$ & $25.74\pm43.23$ \\
CLPU-DER++$^\ddagger$ & buffer (600) + model copy & $65.81\pm1.25$ & $-15.63\pm1.82$ & $0.00\pm0.00$ & $0.00\pm0.00$ \\
\textbf{LwU} & $\mathcal{D}'_r$ (2,480) & \textbf{73.65$\pm$1.13} & \textbf{-1.45$\pm$0.67} & \textbf{0.00$\pm$0.00} & \textbf{0.00$\pm$0.00} \\
LwU, request-time $\mathcal{D}'_r$ & none from tasks 1--2 & $72.55\pm1.51$ & $-2.73\pm0.74$ & $0.00\pm0.00$ & $0.00\pm0.00$ \\
LwU, $\mathcal{D}'_r$ = 1\% & $\mathcal{D}'_r$ (248) & $71.80\pm1.52$ & $-3.90\pm0.98$ & $0.00\pm0.00$ & $0.00\pm0.00$ \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}

The default LwU setting reaches 73.65\% ACC and a final deleted-class accuracy of zero, compared with 69.94\% ACC for LwF+SalUn and 65.81\% for CLPU-DER++. The request-time-only $\mathcal{D}'_r$ variant reaches 72.55\% ACC and also leaves the deleted class at zero. The difference between default and request-time retention partly reflects the availability of historical images, so the default should not be described as fully replay-free at deletion.

\begin{table*}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{3pt}
\caption{Retain-set provenance controls under the five-task joint protocol. The request-time variant has no images from tasks 1--2. Three seeds.}
\label{tab:new_request_subset}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{lcccc}
\toprule
LwU setting & Images of tasks 1--2 stored & ACC $\uparrow$ & BWT $\uparrow$ & $F_{\mathrm{del}}$ / $F_{\mathrm{end}}$ $\downarrow$ \\
\midrule
No deletion & none & $72.65\pm1.20$ & $-2.78\pm0.32$ & -- \\
\textbf{Deletion, request-time $\mathcal{D}'_r$} & \textbf{none} & \textbf{72.55$\pm$1.51} & \textbf{-2.73$\pm$0.74} & \textbf{0.00 / 0.00} \\
Deletion, $\mathcal{D}'_r$ from tasks 1--3 (default) & yes & $73.65\pm1.13$ & $-1.45\pm0.67$ & $0.00 / 0.00$ \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}

\begin{table*}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{3pt}
\caption{Deletion timing and retain-set sensitivity for LwU on the five-task joint protocol (three seeds). Values are reproduced from the additional experiments.}
\label{tab:new_deletion_schedule}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{lcccc}
\toprule
Setting & ACC $\uparrow$ & BWT $\uparrow$ & $F_{\mathrm{del}}$ $\downarrow$ & $F_{\mathrm{end}}$ $\downarrow$ \\
\midrule
Delete after task 2 & $73.81\pm1.09$ & $-1.59\pm0.47$ & $0.00\pm0.00$ & $0.00\pm0.00$ \\
Delete after task 3 & $73.65\pm1.13$ & $-1.45\pm0.67$ & $0.00\pm0.00$ & $0.00\pm0.00$ \\
Delete after task 4 & $74.12\pm1.32$ & $-0.82\pm0.60$ & $0.00\pm0.00$ & $0.00\pm0.00$ \\
Two requests (after 2 and 4) & $74.28\pm1.11$ & $-1.14\pm0.88$ & $0.00\pm0.00$ & $0.00\pm0.00$ \\
Retain subset 1\% & $71.80\pm1.52$ & $-3.90\pm0.98$ & $0.00\pm0.00$ & $0.00\pm0.00$ \\
Retain subset 5\% & $73.35\pm1.43$ & $-1.69\pm0.72$ & $0.00\pm0.00$ & $0.00\pm0.00$ \\
Retain subset 25\% & $73.75\pm1.02$ & $-1.17\pm0.87$ & $0.00\pm0.00$ & $0.00\pm0.00$ \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}

The 20-task study uses 20 tasks of five classes, with requests after tasks 5, 10, and 15. All methods use the same settings selected in the five-task study; they are not re-tuned for the longer stream. In this harder stream LwU retains strong deletion outcomes but underperforms the replay-based baselines in ACC. Individual request outcomes should not be substituted for privacy auditing.

\begin{table*}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\caption{Twenty-task Split CIFAR-100 interleaved deletion with three requests. Each deleted-class accuracy tuple is ordered by request 1/2/3. Three seeds.}
\label{tab:new_long_stream}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{lccccc}
\toprule
Method & Knows requests in advance & ACC $\uparrow$ & BWT $\uparrow$ & $F_{\mathrm{del}}$ r1 / r2 / r3 $\downarrow$ & $F_{\mathrm{end}}$ r1 / r2 / r3 $\downarrow$ \\
\midrule
LwF + SalUn & no & $79.24\pm3.68$ & $-7.20\pm2.02$ & $8.78 / 17.09 / 28.45$ & $2.01 / 28.25 / 12.13$ \\
CLPU-DER++ & yes & $81.22\pm1.73$ & $-6.31\pm0.58$ & $0.00 / 0.00 / 0.00$ & $0.00 / 0.00 / 0.00$ \\
LwU & no & $74.71\pm1.17$ & $-7.79\pm0.51$ & $0.00 / 0.00 / 3.98$ & $0.00 / 0.00 / 3.06$ \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}

\subsubsection{Mechanism ablations in the joint stream}
These ablations distinguish the role of the four-zone updates from the empirical Fisher estimator itself. The dominance margin and self-distillation teacher have the largest impacts on accuracy. Omitting Zone B reset increases the deleted-class accuracy even when it leaves average CL accuracy nearly unchanged.

\begin{table}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{3pt}
\caption{Continual-learning-only ablations on five-task Split CIFAR-100; no deletion (three seeds).}
\label{tab:new_cl_only_ablation}
\begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{lcc}
\toprule
Variant & ACC $\uparrow$ & BWT $\uparrow$ \\
\midrule
w/o self-distillation teacher & $45.78\pm1.52$ & $-36.72\pm0.55$ \\
w/o cumulative freeze mask & $72.00\pm1.48$ & $-5.75\pm1.43$ \\
\textbf{LwU} & \textbf{72.65$\pm$1.20} & \textbf{-2.78$\pm$0.32} \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}

\begin{table*}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{3pt}
\caption{Five-task joint CL--MU component ablations on Split CIFAR-100; deleted class requested after task 3 (three seeds).}
\label{tab:new_joint_ablation}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{lcccc}
\toprule
Variant & ACC $\uparrow$ & BWT $\uparrow$ & $F_{\mathrm{del}}$ $\downarrow$ & $F_{\mathrm{end}}$ $\downarrow$ \\
\midrule
No dominance margin ($\omega=1$) & $34.15\pm0.65$ & $-45.08\pm0.59$ & $0.00\pm0.00$ & $0.00\pm0.00$ \\
w/o self-distillation teacher & $48.80\pm2.95$ & $-32.91\pm3.45$ & $0.00\pm0.00$ & $0.00\pm0.00$ \\
w/o teacher repair & $71.12\pm1.56$ & $-4.54\pm1.27$ & $6.05\pm3.86$ & $8.41\pm8.14$ \\
w/o Zone B reset & $73.84\pm1.05$ & $-1.31\pm0.58$ & $7.69\pm10.10$ & $2.87\pm4.31$ \\
w/o Zone-C repair pass & $73.01\pm0.81$ & $-2.15\pm0.56$ & $0.00\pm0.00$ & $0.00\pm0.00$ \\
w/o cumulative freeze mask & $73.97\pm0.12$ & $-3.30\pm0.13$ & $0.00\pm0.00$ & $0.00\pm0.00$ \\
\textbf{LwU} & \textbf{73.65$\pm$1.13} & \textbf{-1.45$\pm$0.67} & \textbf{0.00$\pm$0.00} & \textbf{0.00$\pm$0.00} \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}

\subsection{Unified U-LiRA Privacy Audit}\label{sec:new_unified_privacy}
The former summary table and ROC plots used incompatible instance-deletion audit settings. We therefore restrict comparable privacy results to one protocol: 16 retrained shadow models, 4,500 deleted images for instance deletion, and seed 42. AUC of 50\% is chance-level distinguishability; lower TPR at 1\% FPR is desirable. These privacy results are not pooled with forget-accuracy or legacy attack metrics to award overall medals. Class-deletion results below are from a separate standalone class-deletion evaluation. Under the unified audit LwU reduces leakage relative to Original in all eight reported instance/class cells, but does not consistently achieve Retrain-level privacy.

\begin{table*}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{3pt}
\caption{Protocol-consistent standalone instance deletion U-LiRA (seed 42, 16 shadows, 4,500 forget images). AUC and TPR are percentages.}
\label{tab:new_privacy_instance}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{lccc}
\toprule
Setting & Original AUC & LwU AUC & LwU TPR@1\% FPR \\
\midrule
CIFAR-10, CNN & $66.78$ & $62.52$ & $8.80$ \\
CIFAR-10, ResNet-18 & $80.08$ & $77.72$ & $20.29$ \\
CIFAR-100, CNN & $81.78$ & $76.48$ & $15.76$ \\
CIFAR-100, ResNet-18 & $93.05$ & $84.23$ & $38.11$ \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}

\begin{table*}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{3pt}
\caption{Standalone class deletion U-LiRA under the reported consistent class-deletion audit. AUC and TPR are percentages.}
\label{tab:new_privacy_class}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{lccc}
\toprule
Setting & Original AUC & LwU AUC & LwU TPR@1\% FPR \\
\midrule
CIFAR-10, CNN & $100.00$ & $73.28$ & $31.96$ \\
CIFAR-10, ResNet-18 & $100.00$ & $53.38$ & $0.31$ \\
CIFAR-100, CNN & $100.00$ & $61.63$ & $4.67$ \\
CIFAR-100, ResNet-18 & $100.00$ & $60.64$ & $0.22$ \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}

\subsection{Deletion, Repair, and Subsequent Learning}\label{sec:new_repair_trajectory}
We examine four ways to repair after the same destructive edit: (i) pre-edit masked teacher (standard LwU), (ii) oracle Retrain teacher as a diagnostic only, (iii) cross-entropy without a teacher, and (iv) edit-anchored repair. Stage-wise U-LiRA used 16 shadow streams per seed over three seeds. Where the source reports a single number or a pair without a standard deviation, we do not impute uncertainty. The precise edit-anchored optimization rule is not supplied with these numerical records and must be added before a reproducibility claim is made.

\begin{table*}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{3pt}
\caption{Class-deletion trajectory on five-task Split CIFAR-100 with class masking. End means after tasks 4--5; paired values follow after-repair/end order. Deleted and retained accuracies are percentages.}
\label{tab:new_class_repair}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{lcccc}
\toprule
Repair & Stage & U-LiRA AUC & Deleted acc & Retained acc \\
\midrule
none & before request & $83.61\pm15.97$ & $70.19$ & $71.61$ \\
none & after edit & $62.09\pm6.07$ & $12.47$ & $69.51$ \\
\textbf{LwU (pre-edit teacher)} & after repair & \textbf{48.36$\pm$5.44} & $0.00$ & $73.14$ \\
\textbf{LwU (pre-edit teacher)} & after tasks 4--5 & \textbf{47.75$\pm$5.47} & $0.00$ & $72.57$ \\
Oracle teacher & after repair / end & $48.27 / 48.54$ & $0.00$ & $73.49 / 72.52$ \\
No teacher & after repair / end & $59.27 / 59.28$ & $0.00 / 0.51$ & $73.33 / 73.19$ \\
Edit-anchored repair & after repair / end & $56.60 / 50.86$ & $0.00$ & $71.64 / 71.61$ \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}

With a class mask, standard LwU produces a U-LiRA AUC of $48.36\pm5.44$ immediately after repair and $47.75\pm5.47$ after subsequent tasks, with deleted-class accuracy zero at both stages. In this class-deletion setting, masked pre-edit repair does not show evidence of reinstating the deleted class. This does not extend automatically to instance or subclass deletion: their labels remain active, so no class can be masked.

\begin{table*}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{3pt}
\caption{Participant-deletion proxy: one fine class within a retained CIFAR-20 superclass; no class-logit mask. Stage pairs are after repair/end of task 5. No standard deviation is implied for values reported as pairs.}
\label{tab:new_participant_repair}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{lcccc}
\toprule
Repair & Stage & U-LiRA AUC & Participant acc & Retained acc \\
\midrule
none & before request & $60.35\pm6.31$ & $75.37$ & $82.98$ \\
none & after edit & $48.06\pm4.89$ & $34.65$ & $78.82$ \\
LwU (pre-edit teacher) & after repair / end & $61.42 / 58.71$ & $75.66 / 73.76$ & $83.47 / 83.49$ \\
Oracle teacher & after repair / end & $60.65 / 60.91$ & $71.88 / 74.85$ & $83.45 / 83.52$ \\
No teacher & after repair / end & $60.87 / 57.40$ & $78.26 / 76.64$ & $82.99 / 83.66$ \\
\textbf{Edit-anchored repair} & after repair / end & \textbf{54.12 / 50.47} & $47.53 / 41.00$ & $82.52 / 83.33$ \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}

\begin{table*}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{3pt}
\caption{Participant-proxy deletion after task 3, evaluated over ten seeds. Distance is the absolute difference between participant accuracy and the Retrain reference after task 5.}
\label{tab:new_participant_10seed}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{lcccc}
\toprule
Method & ACC $\uparrow$ & BWT $\uparrow$ & Participant acc after task 5 & Distance to Retrain $\downarrow$ \\
\midrule
Retrain (never sees the participant) & $83.34\pm1.01$ & $-1.48$ & $56.39\pm29.14$ & -- \\
LwU (pre-edit teacher) & $83.91\pm0.62$ & $-1.38$ & $78.76\pm14.42$ & $22.4$ \\
\textbf{LwU, edit-anchored repair} & $83.12\pm1.38$ & $-2.34$ & $41.74\pm22.87$ & $14.7$ \\
LwU, edit only & $80.23\pm2.69$ & $-6.00$ & $29.45\pm26.26$ & $26.9$ \\
LwF + SalUn & $83.64\pm1.15$ & $-4.35$ & $46.58\pm19.94$ & $9.8$ \\
CLPU-DER++ & $77.71\pm1.63$ & $-12.10$ & $34.63\pm26.52$ & $21.8$ \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}

Without a class mask, standard repair returns participant accuracy toward its pre-request value and U-LiRA AUC to about 60. The oracle teacher shows similar behavior, indicating that repair on retained inputs sharing the participant label also contributes. Edit-anchored repair reduces final AUC to 50.47 in the reported trajectory, but its 10-seed mean participant-accuracy distance to Retrain (14.7 points) remains larger than LwF+SalUn's (9.8 points). This proxy is not an RTI patient-level privacy demonstration.

For standalone instance and subclass deletion (seed 42, 16 shadows), the oracle teacher's AUC differs from the pre-edit teacher by at most two points in six of eight settings. On ResNet-18 instance deletion, the oracle produces a lower AUC by 8.3 points on CIFAR-10 (70.3 versus 78.6 in the recomputed analysis) and 4.1 points on CIFAR-100 (80.1 versus 84.2). A teacher-dependent contribution is thus measurable, but remains distinct from leakage caused by retained-data repair. No full uncertainty estimates were supplied for these eight comparisons.

\subsection{Additional CIFAR-100 Unlearning Ablations}\label{sec:new_cifar100_ablation}
The following experiments use three seeds. The reported Gap is the mean absolute difference from Retrain across Forget, Retain, and the conventional MIA metric; it is not U-LiRA AUC. Relearn@1 denotes forget-set accuracy after one epoch on the forget set and an equal number of retained examples. Class-deletion ablations are shown on both CNN and ResNet-18; an additional subclass experiment deletes the apple subclass on CNN.

\begin{table*}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\caption{CIFAR-100 class-deletion component ablation on CNN; three seeds. The Gap and MIA columns use the evaluation in the supplied ablation records, not the U-LiRA protocol.}
\label{tab:new_c100_cnn_class}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{lcccccc}
\toprule
Variant & Forget $\downarrow$ & Retain $\uparrow$ & Test $\uparrow$ & MIA & Gap $\downarrow$ & Relearn@1 $\downarrow$ \\
\midrule
Original & $83.00\pm3.61$ & $66.15\pm0.31$ & $66.32\pm0.28$ & $56.96\pm1.68$ & $29.86\pm1.17$ & $95.67\pm1.15$ \\
Retrain & $0.00\pm0.00$ & $66.82\pm0.47$ & $66.15\pm0.46$ & $51.05\pm2.46$ & $0.00$ & $0.00\pm0.00$ \\
w/o Zone B reset & $6.33\pm4.51$ & $66.54\pm0.20$ & $65.94\pm0.25$ & $55.48\pm3.27$ & $3.74\pm1.32$ & $96.00\pm1.73$ \\
w/o teacher repair & $20.67\pm26.10$ & $61.02\pm2.70$ & $60.62\pm2.44$ & $51.34\pm1.03$ & $9.64\pm9.69$ & $89.33\pm13.28$ \\
\textbf{LwU} & \textbf{0.00$\pm$0.00} & \textbf{66.29$\pm$0.17} & \textbf{65.63$\pm$0.17} & \textbf{48.60$\pm$4.06} & \textbf{1.38$\pm$0.56} & \textbf{0.00$\pm$0.00} \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}

\begin{table*}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\caption{CIFAR-100 class-deletion component ablation on ResNet-18; three seeds. Relearn@1 is after one epoch.}
\label{tab:new_c100_resnet_class}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{lcccccc}
\toprule
Variant & Forget $\downarrow$ & Retain $\uparrow$ & Test $\uparrow$ & MIA & Gap $\downarrow$ & Relearn@1 $\downarrow$ \\
\midrule
Original & $85.67\pm3.06$ & $70.16\pm0.44$ & $70.31\pm0.42$ & $63.61\pm1.99$ & $33.60\pm1.47$ & $92.00\pm1.00$ \\
Retrain & $0.00\pm0.00$ & $70.23\pm0.48$ & $69.53\pm0.47$ & $48.61\pm0.90$ & $0.00$ & $0.00\pm0.00$ \\
w/o Zone B reset & $65.33\pm4.16$ & $70.30\pm0.41$ & $70.25\pm0.37$ & $63.38\pm3.87$ & $26.77\pm0.53$ & $94.33\pm1.53$ \\
w/o teacher repair & $1.00\pm1.73$ & $64.05\pm3.87$ & $63.42\pm3.85$ & $50.48\pm6.36$ & $3.80\pm0.83$ & $81.33\pm16.77$ \\
\textbf{LwU} & \textbf{0.00$\pm$0.00} & \textbf{69.68$\pm$0.73} & \textbf{68.99$\pm$0.72} & \textbf{50.86$\pm$2.33} & \textbf{0.96$\pm$0.76} & \textbf{0.00$\pm$0.00} \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}

\begin{table*}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{3pt}
\caption{CIFAR-100 apple subclass deletion on CNN; three seeds. Forget accuracy is compared with Retrain's nonzero target rather than minimized.}
\label{tab:new_c100_cnn_subclass}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{lcccc}
\toprule
Variant & Forget & Retain $\uparrow$ & MIA & Gap $\downarrow$ \\
\midrule
Original & $95.00\pm1.00$ & $77.82\pm0.51$ & $51.25\pm5.44$ & $4.22\pm0.87$ \\
Retrain & $90.67\pm2.31$ & $78.04\pm0.57$ & $46.90\pm4.55$ & $0.00$ \\
w/o Zone B reset & $94.67\pm0.58$ & $77.94\pm0.49$ & $51.27\pm5.31$ & $4.07\pm1.05$ \\
w/o teacher repair & $32.00\pm55.43$ & $71.47\pm6.48$ & $48.98\pm3.31$ & $24.46\pm18.50$ \\
w/o Zone-C step & $92.67\pm3.06$ & $77.22\pm0.41$ & $47.28\pm1.51$ & $2.76\pm0.55$ \\
w/o C projection & $91.00\pm4.58$ & $77.10\pm0.40$ & $47.56\pm2.85$ & $2.74\pm1.08$ \\
w/o Zone-C repair pass & $87.33\pm9.07$ & $76.75\pm0.64$ & $46.18\pm1.28$ & $4.09\pm0.34$ \\
w/o test-time memory & $92.33\pm2.31$ & $77.12\pm0.43$ & $47.39\pm2.40$ & $2.60\pm0.79$ \\
+ weight alignment & $93.00\pm2.00$ & $77.08\pm0.34$ & $47.71\pm1.69$ & $2.68\pm0.36$ \\
\textbf{LwU} & \textbf{92.33$\pm$2.31} & \textbf{77.16$\pm$0.38} & \textbf{47.52$\pm$2.15} & \textbf{2.55$\pm$0.75} \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}

\subsection{Test-Time Memory Latency}\label{sec:new_latency}
The latency benchmark measures batch-size-one ResNet-18 inference at $32\times32$ resolution on an NVIDIA RTX PRO 6000, with every example written to memory and otherwise idle GPU. Deletion runs outside the haptic control loop. Sync-free and compiled versions remove host--device synchronization overhead; the reported outputs agree within $10^{-7}$. This measurement does not establish end-to-end network or robotic-control-loop latency.

\begin{table}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{3pt}
\caption{Inference latency at batch size 1 on RTX PRO 6000, ResNet-18 ($32\times32$); milliseconds per sample.}
\label{tab:new_latency}
\begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{lc}
\toprule
Setting & ms per sample \\
\midrule
Backbone (= LwU with memory off) & $0.57$ \\
LwU + memory, submitted code & $1.07$ \\
LwU + memory, sync-free (identical outputs) & $0.77$ \\
\textbf{LwU + memory, sync-free, compiled} & \textbf{0.57} \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}


